Search for supersymmetry in events with large missing transverse momentum, jets, and at least one tau lepton in 20 fb$^{-1}$ of $\sqrt{s}$=8 TeV proton-proton collision data with the ATLAS detector

A search for supersymmetry (SUSY) in events with large missing transverse momentum, jets, at least one hadronically decaying tau lepton and zero or one additional light leptons (electron/muon), has been performed using 20.3 fb$^{-1}$ of proton-proton collision data at $\sqrt{s} = 8$ TeV recorded with the ATLAS detector at the Large Hadron Collider. No excess above the Standard Model background expectation is observed in the various signal regions and 95% confidence level upper limits on the visible cross section for new phenomena are set. The results of the analysis are interpreted in several SUSY scenarios, significantly extending previous limits obtained in the same final states. In the framework of minimal gauge-mediated SUSY breaking models, values of the SUSY breaking scale $\Lambda$ below 63 TeV are excluded, independently of tan$\beta$. Exclusion limits are also derived for an mSUGRA/CMSSM model, in both the R-parity-conserving and R-parity-violating case. A further interpretation is presented in a framework of natural gauge mediation, in which the gluino is assumed to be the only light coloured sparticle and gluino masses below 1090 GeV are excluded.

==> generatortable.tex <==
\begin{tabular}{l|c|c|c|c}
  \hline
  \hline
	Process & Generator + frag./had. & cross section & underl. event & PDF set \\
  \hline
  $W$,\,$Z$+jets & \Sherpa 1.4.1 & -- &  ??? & \CT10 \\
  $W$,\,$Z$+jets (syst.) & \Alpgen~2.14
Trigger selection&\multicolumn{2}{|c}{$\LJetPt > \GeV{130}$, $\SLJetPt > \GeV{30}$}\\
		&\multicolumn{2}{|c}{$\met>\GeV{150}$}\\
		\hline
Taus		&\multicolumn{2}{|c}{$N_\tau^\text{medium}=1$}\\
         &\multicolumn{2}{|c}{$\pT>30$\,GeV}\\
        \hline
Light leptons	&\multicolumn{2}{|c}{$N_\ell^\text{baseline}=0\qquad$}\\
		\hline % &&&\\
QCD rejection	&\multicolumn{2}{|c}{$ \Delta\phi(\text{jet}_{1,2},\met) > 0.4 $, $ \Delta \phi(\tau,\met) > 0.2 $}\\
			
	    \hline
Signal cuts	&\multicolumn{2}{|c}{$\mT > 140\GeV$}\\
		&$\met > 200\GeV$&$\met > 300\GeV$\\
		&$\HT > 800\GeV$&$\HT > 1000\GeV$\\
\hline

 \end{tabular}
\vspace{40pt}

%  \centering
 \begin{tabular}{l|c|c|c|c}
  \hline
  \hline
			&\twotau Inclusive SR&\twotau bRPV SR&\twotau nGM SR&\twotau GMSB SR\\
  \hline
Trigger selection&\multicolumn{4}{|c}{$\LJetPt > \GeV{130}$, $\SLJetPt > \GeV{30}$}\\
		&\multicolumn{4}{|c}{$\met>\GeV{150}$}\\
		\hline
Taus		&\multicolumn{4}{|c}{$N_\tau^\text{loose}\geq2$}\\
         &\multicolumn{4}{|c}{$\pT>20$\,GeV} \\
        \hline
Light leptons	&\multicolumn{4}{|c}{$N_\ell^\text{baseline}=0\qquad$}\\
		\hline % &&&\\
QCD rejection	&\multicolumn{4}{|c}{$\Delta\phi(\text{jet}_{1,2},\met)\geq 0.3$}\\
			
	    \hline
Signal cuts	&\multicolumn{2}{|c}{$\mTT\geq \GeV{150}$}&\multicolumn{2}{|c}{$\mTT\geq \GeV{250}$}\\
\cline{2-5}
		&$\HT > 600\GeV$&$\HT > 1000\GeV$&$\HT > 600\GeV$&$\HT > 1000\GeV$\\
		&&$\njet\geq4$&$\njet\geq4$&$\njet\geq4$\\
\hline

 \end{tabular}
\vspace{40pt}


 \begin{tabular}{l|c|c|c|c}
  \hline
  \hline
  &\tauleps GMSB SR&\tauleps nGM SR & \tauleps bRPV SR & \tauleps mSUGRA SR\\
  \hline
  Trigger selection&\multicolumn{4}{|c}{$p_\text{T}^\ell>\GeV{25}$}\\
  \hline
  Taus &\multicolumn{4}{|c}{$N_\tau^\text{loose}\geq1$}\\
  & \multicolumn{4}{|c}{$\pT>20$\,GeV} \\
  \hline
  Light leptons	&\multicolumn{4}{|c}{$N_\ell^\text{signal}=1,\quad N_\text{other lep}^\text{baseline}=0$}\\
  \hline % &&&\\
  QCD rejection 	&\multicolumn{4}{|c}{$m_\text{T}^\ell >$ 100 GeV}\\
\hline
   Signal cuts & $\meff > \GeV{1700}$ & $\met >\GeV{350}$&$\meff>\GeV{1300}$& $\met >\GeV{300}$\\
   & & $N_\text{jet}\geq3$&$N_\text{jet}\geq4$&$N_\text{jet}\geq3$\\

  \hline


 \end{tabular}
% \vspace{40pt}
%  
%  \begin{tabular}{l|ccc}
%  \hline
%  \hline
%  \twotau SR		& \HT Cut	& \mTT Cut	& \njet Cut	\\
%  \hline
% %  Inclusive	& $>\GeV{1000}$	& $>\GeV{150}$	& --		\\
%  GMSB		& $>\GeV{1000}$	& $>\GeV{250}$	& $\geq4$	\\
%  nGM		& $>\GeV{600}$	& $>\GeV{250}$	& $\geq4$	\\
%  bRPV		& $>\GeV{1000}$	& $>\GeV{150}$	& $\geq4$	\\
% %  bRPV \moh	& $>\GeV{1000}$	& $>\GeV{150}$	& $\geq4$	\\
% %  bRPV \mz	& $>\GeV{600}$	& $>\GeV{200}$	& $\geq4$	\\
%  \hline
%  \hline
% \end{tabular}
% 


==> resulttable_hadronic.tex <==
\input{resulttable_onetau}

\input{resulttable_twotau}

==> resulttable_semilep.tex <==
\input{resulttable_tauel}

\input{resulttable_taumu}


==> section_signal_effs.tex <==
%The simulated signal samples for the SUSY models considered in this paper have been described in \sect~\ref{sec:SimulatedSamples}. 
%The total cross section for the GMSB model drops from 
%$\unit[100]{pb}$ for $\Lambda = \unit[15]{TeV}$ to 
%$\unit[37]{pb}$ for $\Lambda = \unit[40]{TeV}$ to 
%$\unit[5.0]{fb}$ for $\Lambda = \unit[80]{TeV}$ 
%$\unit[2.0]{fb}$ for $\Lambda = \unit[100]{TeV}$ 

In the GMSB signal scenario, the strong production cross section for 
which the analyses have the largest sensitivity
decreases faster with increasing $\Lambda$ than the cross section for slepton 
and gaugino production. Therefore, the selection efficiency with 
respect to the total SUSY production decreases for large values of $\Lambda$. 

For high $\tan\beta$ the acceptance times efficiency is of the order of 0.3\% for the \onetau channel, 0.5\% for the \twotau channel. 
For low $\tan\beta$ those values drop to 0.1\% for the \onetau channel and 0.2\% for the \twotau channel. For the \taulep channel the acceptance
times efficiency varies between 0.2\% to 0.4\% across the ($\lambda$, $\tan\beta$) plane.

% in the area where the limit is set. For low $\tan\beta$ values, it drops to 0.1\%. 
%For large $\Lambda$ it rises to values of 10\%.
%For the \twotau channel in the high $\tan\beta$ region the acceptance times efficiency is of the order of 0.5\% and drops to 0.2\% for low $\tan\beta$ values. For the \taulep channels it is about 0.2--0.4\%.

The total systematic uncertainty on the signal selection from the various sources discussed in \sect~\ref{sec:syst} is between 
5--10\% for the \onetau channel, raising up to 20\% for high values of $\Lambda$. 
For the \twotau channel it amounts to 20--30\% for most of the parameter space, increasing to up to 45\% for the region of highest $\Lambda$ and low $\tan\beta$.
For the \taulep channel typical systematics are around 5\% to 15\%.
%

In the mSUGRA signal plane the acceptance times efficiency for the \onetau channel ranges
from permille level to around 4\%, with the higher values being observed in the low $m_{1/2}$ region.
%
The \twotau channel has extremely small acceptance due to the request of the second
high-\pt ~tau, and therefore is not interpreted in this scenario.
%%
The \taulep channels have an acceptance times efficiency range starting
at the permille level and reaching up to 2\%. 
%for the \tauel final state.
The total systematic uncertainty on the signal selection 
%from the various sources discussed in \sect~\ref{sec:syst} 
is at the level
of 10\% across most of the plane for all channels.
% It rises up to 50\% at the lowest $m_{1/2}$ region studied and up to 80\%
% for individual signal points at the highest $m_{1/2}$ values.

In the nGM scenario only
the gluino pair production is considered. 
The gluino pair production cross section is primarily a function of $m_{\tilde{g}}$, ranging from $\unit[17.2]{pb}$ for $m_{\tilde{g}}=400$~GeV to 
$\unit[7]{fb}$ for $m_{\tilde{g}}=1100$~GeV. 
The \onetau channel does not contribute to the nGM scenario where by construction each event contains at least two taus.
The acceptance times efficiency for the \twotau analysis is at the order of 4\% for high $m_{\tilde{g}}$, independent of 
$m_{\tilde{\tau}}$, and it drops to $\sim$2\% for low $m_{\tilde{g}}$. 
The total experimental systematic uncertainty on the signal selection 
%from the various sources discussed in \sect~\ref{sec:syst} 
is between 
10--20\%.
In the \taulep channels the acceptance times efficiency is in the order of 2\% for high $m_{\tilde{g}}$ and drops to 0.2\% for lower masses. The systematic uncertainties amount to 15--20\% for lower masses
and decreases to an average level of 5--10\% for high $m_{\tilde{g}}$.
%

In the bRPV signal plane the acceptance times efficiency ranges
from the permille level to around 1\% for the \onetau and \twotau
channels (tight SR), with the higher values being observed in the low
$m_0$, high $m_{1/2}$ region.
%
The \taulep channels have an acceptance times efficiency range starting
at the permille level and reaching up to 2\%.
The total systematic uncertainty on the signal selection 
%from the various sources discussed in \sect~\ref{sec:syst} 
is at the level of 10\%
across most of the plane for all channels.
% It rises up to 50\% at the lowest $m_{1/2}$ region studied and up to 80\% for individual signal points at the highest $m_{1/2}$ values.

%Theoretical uncertainties related to the GMSB cross section predictions are
%obtained using the same procedure as detailed in \refer~\cite{combinedtaupaper}.
The nominal cross sections and uncertainties in the different models
discussed in this paper are taken from an envelope of cross section
predictions using different PDF sets and factorization and renormalization
scales, as described in \refer~\cite{Kramer:2012bx}. 
%This procedure is the same
%as detailed in \refer~\cite{ATLAS:SusyTau5fb}
%%
The uncertainties are calculated for individual SUSY production
processes and for each model point in the GMSB, nGM, bRPV and mSUGRA planes.
The overall theoretical cross section uncertainties are between
15--30\% in GMSB, 15--40\% in nGM, 12--20\% in bRPV and 15--35\% in mSUGRA.


